Biases in the Facebook News Feed: a Case Study on the Italian Elections

Facebook News Feed personalization algorithm has a significant impact, on a daily basis, on the lifestyle, mood and opinion of millions of Internet users. Nonetheless, the behavior of such algorithms usually lacks transparency, motivating measurements, modeling and analysis in order to understand and improve its properties. In this paper, we propose a reproducible methodology encompassing measurements and an analytical model to capture the visibility of publishers over a News Feed. First, measurements are used to parameterize and to validate the expressive power of the proposed model. Then, we conduct a what-if analysis to assess the visibility bias incurred by the users against a baseline derived from the model. Our results indicate that a significant bias exists and it is more prominent at the top position of the News Feed. In addition, we found that the bias is non-negligible even for users that are deliberately set as neutral with respect to their political views.

==> News_feed_description.tex <==
\section{News Feed Description}

The News Feed is considered the core service of the Facebook, which defines it as: 	\textit{"a personalized, ever-changing collection of photos, links, videos and updates from the family, businesses, public figures, and news sources you've connected to on Facebook"}\cite{News_Feed}. 
The News Feed is further divided into two different versions, the default \textit{top stories} and the \textit{most recent stories} version. According to the Facebook help center, the difference between the two is that \textit{"Top Stories Shows the most popular stories from friends, Pages and groups at the top of your News Feed"}, while the most recent version shows \textit{"stories from friends, Pages and groups in the order that they were posted."} \cite{Facebook_top_stories}. The user can switch between the two modes, but the curious point is that despite the user chooses the most recent stories mode, "News Feed will eventually return to the default Top Stories setting" \cite{Facebook_top_stories}.
\begin{comment}Even in the most recent stories mode, there exists a filter that selects the \textit{"Friends and pages you interact with most"}, so that the feed most users believed to represent every update from every friend in a real-time stream, in fact became an edited one, much like the Top News filter.
\end{comment}



\subsection{Why users should care about the News Feed top stories algorithm?}

Traditional media always curated, and therefore filtered, the information delivered to the audience. According to Chomsky in \cite{chomsky_Manufacturing_Consent},"the media serve, and propagandize on behalf of, the powerful societal interests that control and finance them". The novelty in the Top Stories algorithm is that the curation is personalized to each user. While the traditional media "has a clear editorial position in which people can debate over" \cite{O'Neil:2016:WMD:3002861}, the Top Stories algorithm creates a particular, private and reduced vision of the world. The filtering results in the creation of a bubble \cite{pariser2011filter}, a bundle including only that information believed to match her preferences .

Trapped in filter bubbles, users can not reach a common vision of reality, as it is difficult to understand what each other believe in and why each other has their beliefs. Therefore, the ability to critically understand,  and deal with contrary opinions, especially in the context of public debates, is potentially damaged.

\begin{comment}
Understanding the filtering process is indeed more relevant, specially because people  believe that Facebook is just a media to connect people, they still believe that the platform shared everything they posted with all of their friends. Research conducted in \cite{Eslami2015a} shows that $62,4 \%$ of the participants was unaware of the Top Stories algorithm.  
\end{comment}

\begin{comment}
Facebook personalization algorithms are not yet open to public scrutiny. But the public has the right to demand a transparent disclosure of the rules by which those algorithms silently shape the way we manage information both as individuals and as societies. This is not only valuable for individuals and societies, but also for Facebook itself. In the long run, the effect of those algorithms can potentially disrupt the value underneath Facebook business partnerships with firms. In fact, by tightening users’ preferences, personalization algorithms might actually create a customer type hostile to the advertising and testing of new products that do not fit its identity expectation.
\end{comment}




==> generaloverview.tex <==
\section{Insights about News Feed modelling }
\label{sec:insights}
Next, we introduce some ideas that supports the analytical model introduced in the following section.




\subsection{Analogies between queuing theory, caches and News Feed}
% 
% post = publicação
% publisher = fonte

In online social networks, posts flow through links connecting their members, reaching a targeted set of  News Feed users. Therefore, News Feed is a communication channel between publishers and users.

In the most naive way, posts are organized in a \emph{first in, first out} (FIFO) fashion. The personalization algorithm 
only filters the posts of publisher $j$ at News Feed of $i$, transforming a creation rate of $\Lambda_j$ into an effective arrival rate of $\lambda_{ij}$.

The procedure recently described, is the procedure of a FIFO queue. Therefore, we argue that is natural take advantage of queueing theory results to model News Feed behavior. 

 We also argue that there are a lot of similarities between News Feed and content caches. Both are used to store content useful for users. Due to the finite size, both acts like filters. In general, both store recent content and evicts contents no longer needed by the users. And, at last but not least, both increases the efficiency of the information retrieval of the content stored inside.  

There is a vast literature about caches and queues theory. By making connections between queues, caches and News Feed we can take advantage of the existing results to get insights about News Feeds, which, due to this young age, received less attention from the scientific community than caches and queues. On the opposite direction, we believe that the knowledge obtained studying News Feed might generate new ways of doing 
caching or new applications of content delivery.







%\subsection{\emph{Timelines} são \emph{caches} orientadas a fontes}
\subsection{Are News Feed caches?}

In this work, one of our goals is to learn how to design News Feed taken advantage of the similarities with caches.
However, there exist important differences between News Feeds and caches.

When News Feed users  search for  user-generated content, they  are typically  interested in a class of items related to a given category or  user. This is the main difference between News Feed and caches. For instance, a user might want to read the most recent headlines of her favourite news paper. This is a more flexible request in comparison, for instance, with an user willing to watch the newest episode of her favourite television show. Table~\ref{table:compare} summarizes some differences between caches  and News Feeds. 



Despite the similarities between caches and News Feeds, traditional caching policies are efficient in serving specific requests. On the other hand, News Feed algorithm have to satisfy the users utilities by delivering class based content.  For the reasons discussed above, we claim that News Feed are publisher-driven caches while traditional caches are request-driven caches, therefore, each one ask for its own caching policy.
  
\begin{table}[t]
\centering
\footnotesize
\caption{Comparison between News Feed and caches }
\label{tab:diferences}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{l||l|l}
%\vspace{+0.1 in}
\hline 
 
 & Timelines & Caches \\
\hline
\hline 
%Admission and eviction decisions & Admission and eviction decisions
%after a content is published &  after a content is missed $j$\\
Trigger event  & post publishing & content request\\
\hline 
Insertion and  & after a post creation & after a miss \\
eviction moments & or engagement & \\
 \hline
 %Tempo de vida   & curto & longo \\
 %dos conteúdos & & \\
% \hline
% Cache armazena & múltiplos itens & no máximo uma cópia \\
% & de uma classe  & de cada item \\
 %\hline
 Cache stores & multiple items & at most one copy \\
 & of content from  & of a specific item \\
 & given class & \\
 \hline
 Requests  & general content  &  specific content\\
 arrive for & classes &  items \\
 \hline 
Control & of items by &  of specific content\\ 
occupancy & given publisher & items \\
\hline
\end{tabular} \label{table:compare}
%}
\end{table}

==> medicoes.tex <==
\section{Medições} \label{sec:medicoes}

% A seguir, descrevemos a metodologia de medições realizadas no Facebook.



\paragraph{Obtenção das métricas de interesse}
Usando a infraestrutura do Facebook Tracking Exposed,\footnote{Facebook tracking exposed: \url{https://facebook.tracking.exposed/}} criamos seis usuários virtuais no Facebook. Todos os usuários seguem as mesmas fontes. Entretanto, os usuários possuem diferentes perfis (e.g., um curte  páginas de direita e outro de esquerda).  A cada hora, colhemos as publicações apresentadas na \emph{timeline} de cada usuários. Tais fotografias constituem nossa base de dados.

Cabe destacar que a API do Facebook desde 2015 não oferece os dados acima~\cite{Facebook_API}. Mesmo quando a API era aberta, o Facebook dizia que a informação fornecida pela API não era fidedigna~\cite{Facebook_API_home}.   Utilizamos esta API somente para colhermos informações sobre o número de publicações por fonte.

\paragraph{Métricas de interesse}
Dentre as métricas de interesse, destacamos as seguintes:

\begin{description}
\item[Repercussão (probabilidade de acerto)] de uma fonte é a probabilidade de um usuário efetivamente ler (e possivelmente clicar) em uma publicação. Nesse trabalho, não distinguimos entre probabilidade de acerto e probabilidade de \emph{click}.  A probabilidadde de acerto de uma fonte pode ser dada pela visibilidade ou pela ocupação das postagens desta fonte.
\item[Visibilidade] é a probabilidade de existir uma publicação de uma determinada fonte na \emph{timeline}.
\item[Ocupação] é o número de publicações de uma determinada fonte na \emph{timeline}.
\end{description}

Denotamos por  $\pi_{ij}$  a visibilidade da fonte $j$ na \emph{timeline} do usuário $i$.  Denotamos por $N_{ij}$  o número médio de publicações do \emph{publisher} $j$ na \emph{timeline} de $i$.    Neste trabalho, assumimos que a repercussão de uma fonte pode ser dada  em função da visibilidade  ou da ocupação. A repercussão  igual a visibilidade condiz  com  usuários que eventualmente irão ler uma das  publicações de cada uma das fontes presentes nas $K$ primeiras posições de suas \emph{timelines}.    A repercussão  igual a ocupação, por outro lado, captura o comportamento de usuários  que irão influenciar-se mais por fontes que ocupam mais posições em suas \emph{timelines}, ou seja,  quanto mais posições ocupadas por uma fonte, maior a repercussão da mesma.  

\begin{comment}
No primeiro caso, temos que
\begin{equation}
h^{(v)}_{ij} = \pi_{ij}
\end{equation}
enquanto que no segundo,
\begin{equation}
h^{(o)}_{ij} = E(N_{ij})/K
\end{equation}
\end{comment}





==> modelos.tex <==
\section{Um modelo analítico para  \emph{timelines}}
\label{sec:model}

A seguir, apresentamos o modelo analítico proposto, seguido por sua validação usando dados das eleições italianas de 2018.

\subsection{Descrição do modelo}

% Nesta seção descrevemos dois modelos para \emph{timelines}. O primeiro modelo assume que as mensagens entram e saem da \emph{timeline} na ordem em que elas são geradas. Ele é mais simples porém menos flexível (FIFO). O segundo modelo é mais flexível, assumindo que cada mensagem está associada a um time-to-live (TTL).




% \subsection{Modelo FIFO} 

\label{sec:fifo}

Nesta seção, descrevemos um  modelo analítico para capturar a dinâmica das publicações em uma \emph{timeline}. 

\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{l l}
%\vspace{+0.1 in}
\hline
\hline
Variável  & descrição \\
\hline
$K$ & número de posições de interesse no topo da \emph{timeline} (\emph{top} $K$)\\
$j$ & $j$-ésima fonte  \\
$i$ & $i$-ésimo  cliente (usuário) \\
$\Lambda_j$ & taxa de criação de publicações da fonte $j$\\
$\lambda_{ij}$ & taxa efetiva de chegada de publicações de $j$ na \emph{timeline} de $i$\\
$\lambda_{i,-j}$ & taxa efetiva de chegada de publicações de outras fontes (que não $j$) na \emph{timeline} de  $i$\\
%$\mathbf{\lambda_i}$ & vector of arrival rates of all publishers at $i$\\
$\lambda_i$ & taxa total de chegada na \emph{timeline} de $i$\\
%$\Lambda_{(-j)}$ & total arrival rate of other publishers than $j$\\
%$\mu_i$ & mean timer rate for publisher $j$ contents\\
$T_{ij}$ & valor esperado para tempo de permanência das publicações da fonte $j$ na \emph{timeline} de $i$\\
%$w_{ij}$ & peso associado à fonte $j$ na \emph{timeline} de $i$ \\
%$hi_{ij}$ & taxa de \emph{hit} da fonte $j$ na \emph{timeline} de  $i$\\
$\hat{\pi}_{ij}$ & visibilidade de $j$ medida  na \emph{timeline} de $i$\\
$\pi_{ij}$ & visibilidade segundo modelo \\
$\hat{N}_{ij}$ & ocupação média das publicações da fonte $j$ medida  na \emph{timeline} de  $i$\\
$N_{ij}$ & ocupação média das publicações de $j$ medida  na \emph{timeline} de  $i$ segundo modelo proposto\\
% $H_i^{(t)}$ & entropia do  snapshot colhido no tempo $t$\\
% $R_i^{(t)}$ &  riqueza do  snapshot colhido no tempo $t$\\
%$p_{ij}$ & probability of selecting a post from publisher $j%$ to \\
% & fill a given slot of News Feed of user $i$\\
%$T_j(k)$ & expected busy period when publisher $j$ enter the News Feed in position k \\
%$N$ & contents viewed per snapshot \\
%$w_j$ & weight associated to publisher $j$\\
%$\Omega$ & function domain \\


%$p_{il}$ & probability of a content from publisher $i$ has size $l$ \\
%$b_i,u_i,v_i$ & weights associated to publisher $j$\\
%$C$ & cost function \\
%$\phi$ & maximum publishing rate \\
%$\gamma$ & balance term in cost funtion\\
%$F^{(n)}$ & value of function $F$ at the n-th iteration\\ 
%$q_j$ & price for publisher $j$\\ 
%$S_j$ & desired setpoint of a metric of publisher $j$\\

\hline

\end{tabular}
\caption{Tabela de notação}
\label{tab:notation}
\end{table}

Dividimos os membros das redes sociais virtuais entre fontes e usuários.  Membros que geram conteúdos são fontes, e membros que consomem tais conteúdos são os usuários.    
Ao administrar sua \emph{timeline}, um usuário ou grupo de usuários pode subscrever a fontes, e um subconjunto das publicações destas fontes será exibida na \emph{timeline}.
Note que numa rede em que a maior parte dos conteúdos é gerada pelos próprios usuários (ex., Facebook), o papel de cada usuário dinamicamente muda entre fonte e usuário.

Seja $\mathcal{I}:=\{1, \dots,i,\dots I\}$ o conjunto de usuários em estudo, cada usuário associado a uma \emph{timeline}, e seja  $\mathcal{J}:=\{1, \dots,j,\dots J\}$ o conjunto de fontes. 
Seja $i$ o usuário de interesse, cuja \emph{timeline} desejamos modelar (a notação é sumarizada na Tabela \ref{tab:notation}). 

A fonte $j$ cria publicações segundo um processo Poisson com taxa $\Lambda_j$. Seja $\lambda\pubj \leq \Lambda_j$ a taxa efetiva com que a fonte $j$ alimenta a \emph{timeline} $i$. 
A taxa agregada de publicações chegando na \emph{timeline} do usuário $i$ é dada por
\begin{equation}
\lambda_i=\sum_{j=1}^J \lambda_{ij}
\end{equation} 
A taxa com que publicações de fontes, diferentes de $j$, chegam ao usuário $i$ é
\begin{equation}
\lambda_{i,-j}= \lambda_i-\lambda_{ij}
\end{equation} 

\paragraph{Dinâmica FIFO} % A Figura \ref{fig:News Feed_schema} mostra um diagram esquemático do funcionamento da \emph{timeline} segundo o modelo FIFO. 
Assumimos que cada publicação entra no topo da \emph{timeline}, na posição 1.  Com taxa $\lambda_i$, as publicações tem sua  posição incrementada em uma unidade.  Estamos interessados nas primeiras $K$ posições (slots) da \emph{timeline}. De forma equivalente, assumimos que a \emph{timeline} tem tamanho  $K$.  Uma publicação é removida da \emph{timeline} quando ela passa da posição $K$ para a posição fictícia  $K+1$.

\begin{comment}
\begin{figure}
\begin{center}
\includegraphics[scale=0.5]{Fifo_Timeline_single_size.eps}
\end{center}
\caption{Modelo esquemático para \emph{timeline} do usuário $i$ }
\label{fig:News Feed_schema}
\end{figure}
\end{comment}


\begin{figure}
\begin{center}
\includegraphics[scale=0.6]{Markov_chain.eps}
\end{center}
\caption{CTMC caracterizando o \emph{post} da fonte $j$ na posição mais no topo na \emph{timeline} do usuário $i$. }
\label{fig:CTMC}
\end{figure}

\paragraph{Cadeia de Markov} A seguir, consideramos uma cadeia de Markov para capturar a evolução das publicações  da fonte $j$, na \emph{timeline} do usuário $i$.  O objetivo é calcular a visibilidade e a ocupação de $j$ na  \emph{timeline} do usuário $i$. Por isso, não levamos em conta a posição de cada publicação de $j$ na \emph{timeline} de $i$, mas apenas a posição da publicação mais no topo. Enquanto houver um \emph{post} de $j$ na \emph{timeline} de $i$, a fonte $j$ estará visível.


A Figura \ref{fig:CTMC} mostra uma cadeia de Markov tempo contínuo  (CMTC) cuja variável de estado $X$ representa a posição mais no topo ocupada por uma publicação da fonte $j$. Seja $\tilde{\pi}_{ij}(x)=P(X=x)$.  Com taxa  $\lambda\pubj$, uma publicação de $j$ chega no topo \emph{timeline}.  Com taxa $\lambda_{i,-j}$, uma publicação de outra fonte faz com que as publicações de $j$ sejam movidas para a posição k+1. A fonte  $j$ estará fora da \emph{timeline} se a sua publicação mais no topo encontrar-se na posição fictícia $K+1$.
Logo,
a visibilidade $\pi_{ij}$ é dada por
\begin{equation}
\pi_{ij}=1-\tilde{\pi}_{ij}(K+1)
\end{equation}
\vspace{0.1in}
\begin{proposition} Em uma FIFO \emph{timeline}, 
 a visibilidade da fonte $j$ na \emph{timeline} do usuário $i$ é
\[\pi_{ij}= 1-\bigg(\frac{\lambda_{i,-j}}{\lambda_i}\bigg)^K\]
\label{prop:fifo_newsfeed}
\end{proposition}




\begin{proof}
O resultado segue imediatamente a partir das equações de balanço do sistema, que podem ser derivadas diretamente a partir da Figura~\ref{fig:CTMC}.
\end{proof}

\begin{proposition} Em uma FIFO \emph{timeline}, a ocupação média da fonte $j$ na \emph{timeline} do usuário $i$ é
\begin{equation}
N_{ij}= \frac{\lambda\pubj K}{\lambda_i}
\label{theo:occupancy_fifo}
\end{equation}
\end{proposition}

\begin{proof}
Quando a  $m$-ésima  publicação entra na \emph{timeline} ela fica visível até a chegada do  $(m+K+1)$-ésima publicação. Já que o tempo médio entre chegadas é $1/\lambda_i$, o tempo de residência da $m$-ésima  publicação é $K/\lambda_i$. Em estado estacionário, seja $T_{ij}$ o tempo médio que publicações de $j$ ficam na \emph{timeline} de $i$,  $T_{ij}=K/\lambda_i$.  Pela lei de Little, $N_{ij}= \lambda\pubj T_{ij}=\frac{\lambda\pubj K}{\lambda_i}$.
\end{proof}


\paragraph{Resumo modelo FIFO} O modelo FIFO é um dos modelos analiticamente tratáveis mais simples que se possa conceber para uma \emph{timeline}.  Nesta seção, apresentamos o modelo FIFO e indicamos como ele pode ser usado para derivar a visibilidade e ocupação média de cada fonte em uma \emph{timeline}.  
Em trabalhos futuros, pretendemos considerar modelos alternativos, mais flexíveis, como aqueles baseados em \emph{caches} do tipo TTL.

% Entretanto, ele pode não possuir poder expressivo para capturar todos os cenários de interesse. A seguir, apresentamos uma generalização de tal modelo, que consiste em permitir que cada \emph{post} tenha um time-to-live a ele associado.

\begin{comment}
\subsection{Modelo TTL} \label{sec:ttl}

Nesta seção, consideramos uma \emph{timeline}  em que \emph{posts} estão associados a um time-to-live (TTL).  Sistemas TTL são úteis para armazenar objetos que tem um tempo de validade/expiração \cite{Jung2003a}, como é o caso de muitos \emph{posts} em \emph{timelines} \cite{How_Facebook_NewsFeed_Works}.   

O modelo TTL foi vastamente estudado no contexto de \emph{caches} \cite{Dehghan2016a,Ferragut,Neglia2017, fofack1,tortellimodel}.  Acreditamos que a conexão aqui estabelecida entre \emph{caches}  TTL e  \emph{timelines} permita estender-se  resultados do domínio de \emph{caches} para o domínio de \emph{timelines}.


Numa \emph{timeline} baseada em  TTL, um contador TTL é associado a cada  \emph{post}.  
O contador da fonte $j$ na \emph{timeline} de $i$ é decrementado em intervalos regulares,  de acordo com uma distribuição com média $T_{ij}$. Quando o contador atinge zero, o conteúdo é removido.  Assumimos que a \emph{timeline} tem tamanho infinito.  

A seguir, assumimos que \emph{posts} chegam segundo uma distriubuição Poisson.  Assim, a \emph{timeline} pode ser modelada como uma fila  $M/G/\infty$, e as  métricas de interesse admitem fórmulas fechadas.

% Pela propriedade de PASTA, $h_{ij}$ is equal to the utilization of  $M/G/\infty$ subsystem. With this observation, is possible to make one further definition:


 \end{comment}

 

\begin{comment}
Let $K_{ij}$ be the mean number of contents of publisher $j$ present in News Feed and let $K_i=\sum_{j \in \mathcal{J}} {K_{ij}}$ be the the expected number of contents of all publishers present in the News Feed. 

%Assuming that a user visualizes his News Feed following a Poisson distribution, due to the PASTA property, $h_{ij}$ is equal to the utilization of  $M/G/\infty$ subsystem. With this observation, is possible to make one further definition:



 % Now, we are able to state the following proposition:

\vspace{0.1in}
\begin{proposition}
Em uma \emph{timeline} do tipo TTL, 
 a visibilidade da fonte $j$ na \emph{timeline} do usuário $i$ é
\[ \pi_{ij}=1-e^{- \Lambda_{j} T_{ij}} \]
\label{theo:visibility_general}
\end{proposition}

\begin{proof}

A filtragem de fluxos Poisson gera fluxos também Poisson. Assim,  
o sistema pode ser decomposto em  $J$ sistemas independentes. O resultado segue como consequência da expressão padrão da utilização de uma fila M/G/$\infty$, que é dada por  $e^{-\lambda_{ij} T_j}$  \cite[p.272]{Harchol-Balter2013}.

\end{comment}


\begin{comment}
This decomposition allows the BCMP theorem \cite[p.380]{Harchol-Balter2013}\cite{BCMP}  be applied to the News Feed system. Let the probability of there is no content of publisher $j$ in the cache be defined as $\pi_{jl}(0)$ for each l-sized subsystem.
Thus, the distribution of the number of contents in the News Feed admits a product form solution and the visibility of $j$ is given by the following product:

\begin{equation}
\pi_{j}(0)=\prod_{l=1}^L (\pi_{jl}(0))
\label{eq:visibility_prod_form}
\end{equation}

\end{comment}

 


\begin{comment} 
 
\begin{equation}
\pi_{jl}(0)=e^{-\lambda_{jl} \mu_j}=e^{-p_{jl}\Lambda_j T_j}
\label{eq:mginfty_solution}
\end{equation}


Substituting equation \eqref{eq:mginfty_solution} in equation \eqref{eq:visibility_prod_form}:

\begin{align}
\pi_{j}(0)&=\prod_{l=1}^L (\pi_{jl}(0)) \nonumber \\
&=\prod_{l=1}^L \exp({-p_{jl} \Lambda_j T_j}) \nonumber \\
&=\exp (-\sum_{l=1}^L p_{jl} \Lambda_j T_j) \nonumber \\
&=\exp (-\Lambda_j T_j)
\end{align}


\begin{equation}
\pi_{jl}(0)=e^{-\lambda_{jl}/\mu_j}=e^{-p_{jl}\Lambda_j T_j}
\label{eq:mginfty_solution}
\end{equation}

Substituting equation \eqref{eq:mginfty_solution} in equation \eqref{eq:visibility_prod_form}:

\begin{align}
\pi_{j}(0)&=\prod_{l=1}^L (\pi_{jl}(0)) \nonumber \\
&=\prod_{l=1}^L \exp({-p_{jl} \Lambda_j T_j}) \nonumber \\
&=\exp (-\sum_{l=1}^L p_{jl} \Lambda_j T_j) \nonumber \\
&=\exp (-\Lambda_j T_j) 
\end{align}



Because $\pi_{j}=1-\pi_{j}(0)$, we have :

\begin{equation}
\pi_{j}=1-e^{-\Lambda_j T_j}
\end{equation}
 


Now, the proof is completed
\end{proof}

\end{comment}


\begin{comment}


\begin{figure}
\begin{center}
\includegraphics[scale=0.5]{timeline_decomposition.eps}
\end{center}
\caption{News Feed decomposition in $L$ subsystems }
\label{fig:News Feed_decomposition}
\end{figure}

\end{comment}
 
\begin{comment}

Now, we are able to state the following proposition that provides a formula for 
the occupancy of publisher $j$ in the news feed of $i$:

\vspace{0.1in}
\begin{proposition}
Em uma TTL \emph{timeline}, 
 a ocupação média da fonte $j$ na \emph{timeline} do usuário $i$ é
\[
N_{ij}= \Lambda_{j}  T_{ij}
\]
\label{theo:occupancy}
e
o número médio de slots de interesse ($K$) é igual a \begin{align}
K &=\sum_{j\in\mathcal{J}} N_{ij} \\
\label{eq:K_decomposition}
\end{align}


\end{proposition}   

\begin{proof}


The $M/G/\infty$ assumption allows the poll of posts be decomposed in $|\mathcal{J}|$ independent $M/G/\infty$ subsystems, where $\mathcal{J}:=\{J_1 \cup J_2 \cup \dots \cup J_I\}$.
Therefore, the number of posts of $j$ in the news feed is given by the \textit{Little's Law}.
  
\end{proof}


\end{comment}


\begin{comment}

To model the second stage of the news feed top stories algorithm, we assume that every time a user $i$ access her news feed, a post from publisher $j$ is selected to fill a given slot in the news feed of user $i$ with probability $p_{ij}$ independently of the posts already selected in the previous slots. 

Assuming  that $p_{ij}$ is proportional to the number of posts in the pool weighted by a parameter $w_{ij} \in (0,1)$ that reflects the preference given by the top stories algorithm to the publisher $j$ at user $i$, we have:

\begin{equation}
p_{ij}=w_{ij}\frac{\lambda_{j}T_j}{\sum_{k=1}^J \lambda_{k}T_k}
\label{eq:p_ij_formula}
\end{equation} 

Let us assume that $N$ posts appear in a given snapshot of user $i$. Let $K_{ij}$ be the number of posts of Publisher $j$ at News Feed of $i$ in a given snapshot of $N$ posts. The following proposition, shows the probability of finding $k$ posts in this snapshot.



\begin{proposition}
The distribution of the number of posts of Publisher $j$ at news feed of user $i$ in a given snapshot of $N$ posts is:
\[P[K_{ij}=k]=\binom{N}{k} \bigg(1-w_{ij}\frac{\lambda_{j}T_j}{\sum_{k=1}^J \lambda_{k}T_k}\bigg) ^{N-k} \bigg(w_{ij}\frac{\lambda_{j}T_j}{\sum_{k=1}^J \lambda_{k}T_k}\bigg) ^k \]
\label{prop:dist_binomial}
\end{proposition}  

\begin{proof}

By selecting the posts independently with probability $p_{ij}$, the number of posts of $j$ is given by a binomial distribution with parameter $p_{ij}$ as shown in equation \eqref{eq:binomial_formula}.  

\begin{equation}
P[K_{ij}=k]=\binom{N}{k} (1-p_{ij}) ^{N-k} (p_{ij}) ^k
\label{eq:binomial_formula}
\end{equation}

Substituting equation \eqref{eq:p_ij_formula} in \eqref{eq:binomial_formula} we have proposition \eqref{prop:dist_binomial}.  

\end{proof}


Now, is possible to make one further definition:

\begin{definition}
The visibility of publisher $j$ is given by the steady-state probability $\pi_{ij}$ of finding a content from publisher $j$ in the News Feed of user $i$.
\end{definition}

Now, we are able to state the following proposition:
 
\begin{proposition}
 The visibility of publisher $j$ is given by: 
\[ \pi_{ij}=1-\bigg(1- w_{ij}\frac{\lambda_{j}T_j}{\sum_{k=1}^J \lambda_{k}T_k}\bigg)^N \]
\label{prop:visibility_general}
\end{proposition}

\begin{proof}

Propositon \eqref{prop:visibility_general} can be obtained directly by making $k=0$ in proposition \eqref{prop:dist_binomial}. 


\end{proof}

\end{comment}

\begin{comment}
\subsection{Relacionando os modelos TTL e FIFO}

In a special case where all posts have the same TTL, the TTL news feed behaves like a First-In First-Out (FIFO) system. 
Assuming that users concentrates their attention to the top $K$ positions of the news feed, $K$ can be the desired number of contents in a given news feed. 

By adjusting the TTL timers the expected number of contents in the news feed can be controlled. Alternatively, fixing T, the total arrival rate of posts can be controlled to achieve a desired $K$.
\end{comment}

\begin{comment}
 Section \ref{sec:utility} will provide more sophisticated forms of cache control. This solution will be referred also as absolute egalitarian fairness \cite{moulin_book}.  In this type of control, the visibility is given by the next theorem:
\end{comment}

\begin{comment}
\subsection{Obtaining the visibility and occupancy}




The expect number of slots occupied in news feed $K$ is the sum of $ N_{ij}$:

\begin{align}
K &=\sum_{j\in\mathcal{J}} N_{ij} \\
\label{eq:K_decomposition}
\end{align}

By \textit{Little's Law}, 

\begin{equation}
N_{ij}=\Lambda_j T_{ij}
\label{eq:littles_eq_case}
\end{equation} 

Then,
 
\begin{equation}
K=\sum_{j\in\mathcal{J}} \Lambda_j  T_{ij}
\end{equation}

Because all publishers receive the same treatment, all TTL must be equal. Thus, $T_j=T_{i1}=\dots=T_{1J}$. Therefore,:

\begin{equation}
K =\sum_{j\in\mathcal{J}} \Lambda_j  T_j
\end{equation}

Thus,


\begin{equation}
T = \frac{K}{\sum_j \Lambda_j } =\frac{K}{\Lambda_i }
\label{eq:ttl}
\end{equation}


Substituting the value of T in Proposition \eqref{theo:visibility_general}, we have the following expression for $\pi_{ij}$ :

\begin{equation}
\pi_{ij}=1-\exp\bigg(\frac{-\Lambda_j K}{\Lambda_i}\bigg)
\label{eq:visibility_eq_case}
\end{equation}

Substituting the value of T in Proposition \eqref{theo:occupancy}, we have the following expression for $N_{ij}$ :

\begin{equation}
N_{ij}=\frac{\Lambda_j K}{\Lambda_k}
\label{eq:occupancy_eq_case}
\end{equation}


\end{comment}



